The Role of Diversity in In-Context Learning for Large Language Models

In-context learning (ICL) is a crucial capability of current large language models (LLMs), where the selection of examples plays a key role in performance. While most existing approaches focus on selecting the most similar examples to the query, the impact of diversity in example selection remains underexplored. We systematically investigate the role of diversity in in-context example selection through experiments across a range of tasks, from sentiment classification to more challenging math and code problems. Experiments on Llama-3.1, Gemma-2, and Mistral-v0.3 families of models show that diversity-aware selection methods improve performance, particularly on complex tasks like math and code, and enhance robustness to out-of-distribution queries. To support these findings, we introduce a theoretical framework that explains the benefits of incorporating diversity in in-context example selection.

==> figures/differ-k.tex <==
\begin{figure}
    \centering
    %\begin{subfigure}[t]{\linewidth}
    %\centering
    %\includegraphics[width=0.75\linewidth]{figures/k_classification_comparison.png}
    %\caption{Demonstration set: Amazon, Test set: SST-2}
    %\end{subfigure}
    %\begin{subfigure}[t]{\linewidth}
    %\centering
    %\includegraphics[width=0.75\linewidth]{figures/k_code_length.png}
    %\caption{GeoQuery Length split}
    %\end{subfigure}
    \includegraphics[width=\linewidth]{figures/classification_standard_comparison.png}
    \caption{The performance of different demonstration selection methods with different number of shots $K$. \textbf{Left:} sentiment classification task with demonstrations come from Amazon and queries come from SST-2. \textbf{Right:} text to SQL task with demonstrations and query come from the training and test set of GeoQuery Standard Split.}
    \label{fig:differ-k}
\end{figure}

==> figures/illustration.tex <==
\begin{figure*}[t!]
    \centering
    \begin{subfigure}[t]{0.3\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/topk-illus.pdf}
        \caption{\topk selection}
    \end{subfigure}%
    \begin{subfigure}[t]{0.3\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/div-illus.pdf}
        \caption{\diversity selection}
    \end{subfigure}
    \begin{subfigure}[t]{0.3\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/topk-div-illus.pdf}
        \caption{\topkdiv selection}
    \end{subfigure}
    \caption{An illustrative example for \topk, \diversity, and \topkdiv methods. Point filled in black denotes the query. \textbf{(a)} \topk: Select the most similar demonstrations (3 points filled in red) in the embedding space. \textbf{(b)} \diversity: First select a ``coreset'' based on some \emph{diversity} metric, which is fixed for all queries (6 points filled in gray or red). Then select the most similar demonstrations (3 points filled in red) among this ``coreset''. \textbf{(c)} \topkdiv: Select the demonstrations sequentially based on the linear combination of similarity to the query and the diversity with the selected examples. The first example is the one most similar to the query. When picking the second, it is balanced between the similarity to the query and the diversity from the first example.}
    \label{fig:illustration}
    \vspace{-0.2in}
\end{figure*}

==> figures/knn_diversity_with_k_max.tex <==
\begin{figure}[htbp] % [htbp]
    \centering
    \includegraphics[width=\linewidth, height=5cm]{nips/figures/heatmap_llama-3.2-3b.png}  
    \caption{} 
    \label{fig:knn_diversity_llama-3.2-3b}
\end{figure}

\begin{figure}[htbp]
    \centering

    \includegraphics[width=\linewidth, height=5cm]{nips/figures/heatmap_gemma-2-2b.png}
    \caption{} 
    \label{fig:knn_diversity_gemma-2-2b}
\end{figure}

==> figures/model_size.tex <==
\begin{figure}[!t]
\centering
    \includegraphics[width=0.9\linewidth]{figures/model_size_horizontal.png}
    \caption{\small The relative improvement of diversity-aware methods over \topk.\textbf{ Left:} relative improvement of \topkdiv over \topk on GeoQuery standard split. \textbf{Right:} relative improvement of \diversity over \topk on SCIQ.}
    \label{fig:differ-scale}
\end{figure}

==> figures/various_k.tex <==
\begin{figure}[!t]
\centering
    \includegraphics[width=0.7\linewidth]{figures/sciq_k.png}
    \caption{\textbf{(The accuracy of different methods with different number of shots $K$ on reading comprehension tasks.)} We choose report the results on Llama-3.1-8B, with Sentence-BERT embeddings (all-roberta-large-v1). \textbf{Left:} results where demonstration and query come from SCIQ. \textbf{Right:} results where demonstration and query come from SQuAD.}
    \label{fig:differ-k-sciq}
\end{figure}
